Stacked unsupervised learning with a network architecture found by supervised meta-learning

Stacked unsupervised learning (SUL) seems more biologically plausible than backpropagation, because learning is local to each layer. But SUL has fallen far short of backpropagation in practical applications, undermining the idea that SUL can explain how brains learn. Here we show an SUL algorithm that can perform completely unsupervised clustering of MNIST digits with comparable accuracy relative to unsupervised algorithms based on backpropagation. Our algorithm is exceeded only by self-supervised methods requiring training data augmentation by geometric distortions. The only prior knowledge in our unsupervised algorithm is implicit in the network architecture. Multiple convolutional "energy layers" contain a sum-of-squares nonlinearity, inspired by "energy models" of primary visual cortex. Convolutional kernels are learned with a fast minibatch implementation of the K-Subspaces algorithm. High accuracy requires preprocessing with an initial whitening layer, representations that are less sparse during inference than learning, and rescaling for gain control. The hyperparameters of the network architecture are found by supervised meta-learning, which optimizes unsupervised clustering accuracy. We regard such dependence of unsupervised learning on prior knowledge implicit in network architecture as biologically plausible, and analogous to the dependence of brain architecture on evolutionary history.

==> Invariant Subspace Networks (Arxiv)-9/ablation.tex <==
\begin{table}[t]

% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcc}
\toprule
Experiment & \% Error (test) & \% Error (train) \\
\midrule
4 energy layers & 3.1 & 3.6 \\
3 energy layers & \textbf{2.1} & \textbf{2.5} \\
2 energy layers & 2.9 & 3.3 \\
1 energy layers & 20.2 & 20.7 \\
No ZCA - 3 energy layers & 4.0 & 4.8 \\
No rescaling - 3 energy layers & 4.1 & 4.6 \\
No ZCA \& No rescaling - 3 energy layers& 9.7 & 10.1 \\
1D subspaces - 3 energy layers & 16.0 & 17.3 \\
Random subspaces - 3 energy layers & 29.4 & 31.1\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Systematic studies with our multilayer energy model. The learning hyperparameters are tuned using all 60K labels from the training set.}
\label{tab:ablation}
% \vskip -0.1in
\end{table}


==> Invariant Subspace Networks (Arxiv)-9/comparison.tex <==
\begin{table}[t]

% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lc}
\toprule
representation & clustering error (\%) \\
\midrule
Pixels & 46.2 \\
NMF$^{\ddag}$ \cite{lee1999learning} & 44.0 \\
Stacked Denoising Autoencoders$^{\dagger}$ \cite{vincent2010stacked} & 18.8 \\
UMAP \cite{mcinnes2018umap} & 17.9 \\
Generative adversarial networks$^{\dagger}$ \cite{goodfellow2014generative} & 17.2 \\
Variational autoencoder$^{\dagger}$ \cite{kingma2013auto} & 16.8 \\
Deep Embedded Clustering$^{\dagger}$ \cite{xie2016dec} & 15.7\\
VaDE \cite{jiang2016variational} & 5.5 \\
ClusterGAN$^{\ddag}$ \cite{mukherjee2019clustergan} & 5.0 \\
UMAP + GMM \cite{mcinnes2018umap} & 3.6 \\
N2D \cite{mcconville2021n2d} & 2.1 \\
\textbf{Ours (three layer net)} & \textbf{2.1} \\
Invariant Information Clustering (avg sub-head) $^{\dagger}$ \cite{ji2019invariant} & 1.6\\
Stacked Capsule Autoencoders \cite{kosiorek2019stacked} & 1.3 \\
Invariant Information Clustering (best sub-head)$^{\dagger}$ \cite{ji2019invariant} & 0.8 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Comparison of clustering accuracy for other unsupervised learning algorithms. For methods which do not generate clusters, $k$-means is used to cluster representations into 10 clusters, with the exception of UMAP + GMM in which case we use a Gaussian Mixture Model to cluster. The errors for methods with a dagger $^{\dagger}$ are all taken from \cite{ji2019invariant}, methods with double dagger $^{\ddag}$ are taken from \cite{mukherjee2019clustergan}. UMAP uses ``out-of-the-box'' parameter settings.
\label{tab:comparison}
}
\end{table}

==> Invariant Subspace Networks (Arxiv)-9/data_efficiency.tex <==
\begin{table}[t]

% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{llccccccc}
\toprule
Number of labels in training set & 10 & 30 & 50 & 100 & 500 & 5000 & 60000 \\
\midrule
\% Misclassified (test) & 30.0 & 9.2 & 10.7 & 5.3 & 4.6 & 2.9 & 2.1 \\ 
\% Misclassified (train) & 0.0 & 0.0 & 0.0 & 3.0 & 2.8 & 2.9 & 2.5 \\ 
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Label efficiency of our stacked learning algorithm. In each case, the algorithm has access to all 60K unlabeled images from the training set. What varies is the number of labels we use to evaluate each setting of learning parameters.
\label{tab:data_efficiency}
}
% \vskip -0.1in
\end{table}


==> Invariant Subspace Networks (Arxiv)-9/multilayer_architectures.tex <==
\begin{table*}[t]
\caption{Network architectures for 1,2,3,4 energy layer nets from Table 5.}
\label{tab:multilayer_architectures}
%  \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
Hyperparameter & 1 Layer & 2 Layer & 3 Layer & 4 Layer \\
\midrule
convZCA kernel size & 5 & 9 & 9 & 11\\
convZCA n components & 0 & 18 & 9 & 18\vspace{2mm} \\

layer1 subspace number ($k$) & 59 & 20 & 37 & 15\\
layer1 subspace rank ($r$) & 2 & 5 & 2 & 2\\
layer1 active features ($w$) & 1 & 16 & 9 & 10\\
layer1 kernel size & 10 & 10 & 8 & 7 \\
layer1 padding & 4 & 2 & 2 & 3\vspace{2mm} \\

layer2 subspace number ($k$) & - & 55 & 9 & 63\\
layer2 subspace rank ($r$) & - & 16 & 3 & 12\\
layer2 active features ($w$) & - & 1 & 8 & 1\\
layer2 kernel size & - & 19 & 5 & 17\\
layer2 padding & - & 1 & 1 & 1\vspace{2mm} \\

layer3 subspace number ($k$) & - & - & 58 & 57 \\
layer3 subspace rank ($r$) & - & - & 16 & 7 \\
layer3 active features ($w$) & - & - & 2 & 6 \\
layer3 kernel size & - & - & 21 & 8 \\
layer3 padding & - & - & 2 & 2 \vspace{2mm} \\

layer4 subspace number ($k$) & - & - & - & 22 \\
layer4 subspace rank ($r$) & - & - & - & 1 \\
layer4 active features ($w$) & - & - & - & 1 \\
layer4 kernel size & - & - & - & 3 \\
layer4 padding & - & - & - & 1\vspace{2mm} \\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table*}


==> Invariant Subspace Networks (Arxiv)-9/search_space.tex <==
\begin{table*}[t]
\caption{Hyperparameters that we automatically tune for every network configuration}
\label{search_space}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccccccc}
\toprule
 & \multicolumn{2}{l}{ZCA layer} & \multicolumn{5}{l}{Subspace layers}\\
 & kernel\_size & n\_components & $k$ & $r$ & $p$ & kernel\_size & padding \\

min & 1 & 0 & 2 & 1 & 0 & 1 & 0 \\
max & 11 & kernel\_size & 64 & 16 & $k-2$ & $input\_size$ & $kernel\_size / 2$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table*}

% \begin{table*}[t]
% \caption{Hyperparameters we tune for  for each network configuration}
% \label{sample-table}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{cccccc}
% \toprule
% hyperparam & n subspaces ($n$) & subspace dim ($r$) & sparsity ($p$) & kernel size & padding \\
% min & 2 & 1 & 1 & 1 & 1 \\
% max & 1 & 1 & 1 & 1 & 1 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table*}

==> Invariant Subspace Networks (Arxiv)-9/three_layer_architecture.tex <==
\begin{table}[t]

%  \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccc}
\toprule
Layer & \# subspaces ($k$) & subspace rank ($r$) & \# winners ($w$) & kernel size & padding  \\
\midrule

L1 & 37 & 2 & 9 & 8 & 2 \\
L2 & 9 & 3 & 8 & 5 & 1 \\
L3 & 58 & 16 & 2 & 21 & 2 \\

% layer2 subspace number ($k$) & 9 \\
% layer2 subspace rank ($r$) & 3 \\
% layer2 active features ($w$) & 8 \\
% layer2 kernel size & 5 \\
% layer2 padding & 1\vspace{2mm} \\

% layer3 subspace number ($k$) & 58 \\
% layer3 subspace rank ($r$) & 16 \\
% layer3 active features ($w$) & 2 \\
% layer3 kernel size & 21 \\
% layer3 padding & 2\vspace{2mm} \\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\caption{Detailed architecture of our three energy layer net. The first energy layer is preceded by convolutional ZCA whitening of the input image, where the kernel size is 9 and the number of whitened eigenvalues is 9. These parameters are found with automated hyperparameter tuning.
\label{tab:three_layer_architecture}
}
\end{table}



% % this was intended to be a table with just the architecture of the 3 layer net
% % unfinished

% \begin{table*}[t]
% \caption{Network architecture}
% \label{tab:three_layer_architecture}
% %  \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lc}
% \toprule
% Hyperparameter & Value \\
% \midrule
% convZCA kernel size & 9 \\
% convZCA n components & 9\vspace{2mm} \\

% layer1 subspace number ($k$) & 37 \\
% layer1 subspace rank ($r$) & 2 \\
% layer1 active features ($w$) & 9 \\
% layer1 kernel size & 8 \\
% layer1 padding & 2\vspace{2mm} \\

% layer2 subspace number ($k$) & 9 \\
% layer2 subspace rank ($r$) & 3 \\
% layer2 active features ($w$) & 8 \\
% layer2 kernel size & 5 \\
% layer2 padding & 1\vspace{2mm} \\

% layer3 subspace number ($k$) & 58 \\
% layer3 subspace rank ($r$) & 16 \\
% layer3 active features ($w$) & 2 \\
% layer3 kernel size & 21 \\
% layer3 padding & 2\vspace{2mm} \\

% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table*}


==> Invariant Subspace Networks (Arxiv)-9/three_layer_scores.tex <==
\begin{table}[t]
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccccc}
\toprule
representation & pixels & ZCA & layer 1 & layer 2 & layer 3 & 2x2 pool \\
clustering error (\%) & 46.2 & 50.0 & 22.7 & 22.2 & 2.3 & 2.1 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\caption{Clustering error after every layer of our network with three energy layers.
\label{tab:three_layer_scores}
}
% \vskip -0.1in
\end{table}

% \begin{table*}[t]
% \caption{Clustering error after every layer of our network}
% \label{tab:three_layer_scores}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccccc}
% \toprule
% representation & pixels & ZCA & layer 1 & layer 2 & layer 3 & 2x2 pool \\
% clustering error (\%) & 46.2 & 50.0 & 22.7 & 22.2 & 2.3 & 2.1 \\
% 1NN classifier error (\%) & 62.7 & 63.3 & 44.3 & 39.5 & 5.8 & 4.4 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table*}

==> search_space.tex <==
\begin{table*}[t]
\caption{Hyperparameters that we automatically tune for every network configuration}
\label{search_space}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccccccc}
\toprule
 & \multicolumn{2}{l}{ZCA layer} & \multicolumn{5}{l}{Subspace layers}\\
 & kernel\_size & n\_components & $k$ & $r$ & $p$ & kernel\_size & padding \\

min & 1 & 0 & 2 & 1 & 0 & 1 & 0 \\
max & 11 & kernel\_size & 64 & 16 & $k-2$ & $input\_size$ & $kernel\_size / 2$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table*}

% \begin{table*}[t]
% \caption{Hyperparameters we tune for  for each network configuration}
% \label{sample-table}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{cccccc}
% \toprule
% hyperparam & n subspaces ($n$) & subspace dim ($r$) & sparsity ($p$) & kernel size & padding \\
% min & 2 & 1 & 1 & 1 & 1 \\
% max & 1 & 1 & 1 & 1 & 1 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table*}
